Technical Design Report for the: PANDA Straw Tube Tracker

This document describes the technical layout and the expected performance of the Straw Tube Tracker (STT), the main tracking detector of the PANDA target spectrometer. The STT encloses a Micro-Vertex-Detector (MVD) for the inner tracking and is followed in beam direction by a set of GEM-stations. The tasks of the STT are the measurement of the particle momentum from the reconstructed trajectory and the measurement of the specific energy-loss for a particle identification. Dedicated simulations with full analysis studies of certain proton-antiproton reactions, identified as being benchmark tests for the whole PANDA scientific program, have been performed to test the STT layout and performance. The results are presented, and the time lines to construct the STT are described.

==> authors.tex <==
%
% list of institutions
%
\institem{Universit\"at {\bf Basel}, Switzerland}
\authitem{W.~Erni},
\authitem{I.~Keshelashvili},
\authitem{B.~Krusche},
\authitem{M.~Steinacher}\lastitem
%
\institem{Institute of High Energy Physics, Chinese Academy of Sciences, {\bf Beijing}, China}
\authitem{Y.~Heng},
\authitem{Z.~Liu},
\authitem{H.~Liu},
\authitem{X.~Shen},
\authitem{Q.~Wang},
\authitem{H.~Xu}\lastitem
%
\institem{Universit\"at {\bf Bochum}, I. Institut f\"ur Experimentalphysik, Germany}
\authitem{A.~Aab},
\authitem{M.~Albrecht},
\authitem{J.~Becker},
\authitem{A.~Csap\'o},
\authitem{F.~Feldbauer},
\authitem{M.~Fink},
\authitem{P.~Friedel},
\authitem{F.H.~Heinsius},
\authitem{T.~Held},
\authitem{L.~Klask},
\authitem{H.~Koch},
\authitem{B.~Kopf},
\authitem{S.~Leiber}
\authitem{M.~Leyhe},
\authitem{C.~Motzko},
\authitem{M.~Peliz\"aus},
\authitem{J.~Pychy},
\authitem{B.~Roth},
\authitem{T.~Schr\"oder},
\authitem{J.~Schulze},
\authitem{C.~Sowa},
\authitem{M.~Steinke},
\authitem{T.~Trifterer},
\authitem{U.~Wiedner},
\authitem{J.~Zhong}\lastitem
%
\institem{Rheinische Friedrich-Wilhelms-Universit\"at {\bf Bonn}, Germany}
\authitem{R.~Beck},
\authitem{S.~Bianco},
\authitem{K.T.~Brinkmann},
\authitem{C.~Hammann},
\authitem{F.~Hinterberger},
\authitem{D.~Kaiser},
\authitem{R.~Kliemt},
\authitem{M.~Kube},
\authitem{A.Pitka},
\authitem{T.~Quagli},
\authitem{C.~Schmidt},
\authitem{R.~Schmitz},
\authitem{R.~Schnell},
\authitem{U.~Thoma},
\authitem{P.~Vlasov},
\authitem{D.~Walther},
\authitem{C.~Wendel},
\authitem{T.~W\"urschig},
\authitem{H.G.~Zaunick}\lastitem
%
\institem{Universit\`{a}~di {\bf Brescia}, Italy}
\authitem{A.~Bianconi}\lastitem
%
\institem{Institutul National de C\&D pentru Fizica si Inginerie Nucleara "Horia Hulubei", {\bf Bukarest-Magurele}, Romania}
\authitem{M.~Bragadireanu},
\authitem{M.~Caprini},
\authitem{D.~Pantea},
\authitem{D.~Pantelica},
\authitem{D.~Pietreanu},
\authitem{L.~Serbina},
\authitem{P.D.~Tarta}\lastitem
%
\institem{IIT, Illinois Institute of Technology, {\bf Chicago}, U.S.A.}
\authitem{D.~Kaplan}\lastitem
%
\institem{AGH, University of Science and Technology, {\bf Cracow}, Poland}
\authitem{T.~Fiutowski},
\authitem{M.~Idzik},
\authitem{B.~Mindur},
\authitem{D.~Przyborowski},
\authitem{K.~Swientek}\lastitem
%
\institem{IFJ, Institute of Nuclear Physics PAN, {\bf Cracow}, Poland}
\authitem{B.~Czech},
\authitem{M.~Kistryn},
\authitem{S.~Kliczewski},
\authitem{A.~Kozela},
\authitem{P.~Kulessa},
\authitem{P.~Lebiedowicz},
\authitem{K.~Pysz},
\authitem{W.~Sch\"afer},
\authitem{R.~Siudak},
\authitem{A.~Szczurek}\lastitem
%
\institem{Instytut Fizyki, Uniwersytet Jagiellonski, {\bf Cracow}, Poland}
\authitem{S.~Jowzaee},
\authitem{M.~Kajetanowicz},
\authitem{B.~Kamys},
\authitem{S.~Kistryn},
\authitem{G.~Korcyl},
\authitem{K.~Korcyl},
\authitem{W.~Krzemien},
\authitem{A.~Magiera},
\authitem{P.~Moskal},
\authitem{M.~Palka},
\authitem{Z.~Rudy},
\authitem{P.~Salabura},
\authitem{J.~Smyrski},
\authitem{A.~Wro\'nska}\lastitem
%
\institem{FAIR - Facility for Antiproton and Ion Research in Europe, {\bf Darmstadt}, Germany}
\authitem{I.~Augustin},
\authitem{I.~Lehmann},
\authitem{D.~Nimorus},
\authitem{G.~Schepers}\lastitem
%
\institem{GSI Helmholtzzentrum  f\"ur Schwerionenforschung GmbH, {\bf Darmstadt}, Germany}
\authitem{M.~Al-Turany},
\authitem{R.~Arora},
\authitem{H.~Deppe},
\authitem{H.~Flemming},
\authitem{A.~Gerhardt},
\authitem{K.~G\"otzen},
\authitem{A.F.~Jordi},
\authitem{G.~Kalicy},
\authitem{R.~Karabowicz},
\authitem{D.~Lehmann},
\authitem{B.~Lewandowski},
\authitem{J.~L\"uhning},
\authitem{F.~Maas},
\authitem{H.~Orth},
\authitem{M.~Patsyuk}
\authitem{K.~Peters},
\authitem{T.~Saito},
\authitem{C.J.~Schmidt},
\authitem{L.~Schmitt},
\authitem{C.~Schwarz},
\authitem{J.Schwiening},
\authitem{M.~Traxler},
\authitem{B.~Voss},
\authitem{P.~Wieczorek},
\authitem{A.~Wilms},
\authitem{M.~Z\"uhlsdorf}\lastitem
%
\institem{Veksler-Baldin Laboratory of High Energies (VBLHE), Joint Institute for Nuclear Research. {\bf Dubna},
Russia}
\authitem{V.M.~Abazov}, 
\authitem{G.~Alexeev},
\authitem{A.~Arefiev},
\authitem{V.I.~Astakhov},
\authitem{M.Yu.~Barabanov},
\authitem{B.V.~Batyunya},
\authitem{Yu.I.~Davydov},
\authitem{V.Kh.~Dodokhov},
\authitem{A.A.~Efremov},
\authitem{A.G.~Fedunov},
\authitem{A.A.~Festchenko}, 
\authitem{A.S.~Galoyan},
\authitem{S.~Grigoryan},
\authitem{A.~Karmokov},
\authitem{E.K.~Koshurnikov},
\authitem{V.I.~Lobanov},
\authitem{Yu.Yu.~Lobanov},
\authitem{A.F.~Makarov},
\authitem{L.V.~Malinina},
\authitem{V.L.~Malyshev},
\authitem{G.A.~Mustafaev},
\authitem{A.~Olshevskiy},
\authitem{M.A.~Pasyuk},
\authitem{E.A.~Perevalova},
\authitem{A.A.~Piskun},
\authitem{T.A.~Pocheptsov},
\authitem{G.~Pontecorvo},
\authitem{V.K.~Rodionov},
\authitem{Yu.N.~Rogov},
\authitem{R.A.~Salmin},
\authitem{A.G.~Samartsev},
\authitem{M.G.~Sapozhnikov},
\authitem{G.S.~Shabratova},
\authitem{A.N.~Skachkova}, 
\authitem{N.B.~Skachkov}, 
\authitem{E.A.~Strokovsky},
\authitem{M.K.~Suleimanov},
\authitem{R.Sh.~Teshev},
\authitem{V.V.~Tokmenin},
\authitem{V.V.~Uzhinsky}
\authitem{A.S.~Vodopyanov},
\authitem{S.A.~Zaporozhets},
\authitem{N.I.~Zhuravlev},
\authitem{A.G.~Zorin}\lastitem
%
\institem{University of {\bf Edinburgh}, United Kingdom}
\authitem{D.~Branford},
\authitem{D.~Glazier},
\authitem{D.~Watts},
\authitem{P.~Woods}\lastitem
%
\institem{Friedrich Alexander Universit\"at {\bf Erlangen-N\"urnberg}, Germany}
\authitem{A.~Britting},
\authitem{W.~Eyrich},
\authitem{A.~Lehmann},
\authitem{F.~Uhlig}\lastitem
%
\institem{Northwestern University, {\bf Evanston}, U.S.A.}
\authitem{S.~Dobbs},
\authitem{Z.~Metreveli},
\authitem{K.~Seth},
\authitem{A.~Tomaradze},
\authitem{T.~Xiao}\lastitem
%
\institem{Universit\`{a} di Ferrara and INFN Sezione di Ferrara, {\bf Ferrara}, Italy}
\authitem{D.~Bettoni},
\authitem{V.~Carassiti},
\authitem{A.~Cotta Ramusino},
\authitem{P.~Dalpiaz},
\authitem{A.~Drago},
\authitem{E.~Fioravanti},
\authitem{I.~Garzia},
\authitem{M.~Savri\`e},
\authitem{G.~Stancari}\lastitem
%
\institem{INFN Laboratori Nazionali di {\bf Frascati}, Italy}
\authitem{N.~Bianchi},
\authitem{P.~Gianotti},
\authitem{C.~Guaraldo},
\authitem{V.~Lucherini},
\authitem{D.~Orecchini},
\authitem{E.~Pace}\lastitem
%
\institem{INFN Sezione di {\bf Genova}, Italy}
\authitem{A.~Bersani},
\authitem{G.~Bracco},
\authitem{M.~Macri},
\authitem{R.F.~Parodi}\lastitem
%
\institem{Justus Liebig-Universit\"at {\bf Gie\ss{}en}, II. Physikalisches Institut, Germany}
\authitem{D.~Bremer},
\authitem{V.~Dormenev},
\authitem{P.~Drexler}, 
\authitem{M.~D\"uren},
\authitem{T.~Eissner},
\authitem{K.~F\"ohl}
\authitem{M.~Galuska},
\authitem{T.~Gessler},
\authitem{A.~Hayrapetyan},
\authitem{J.~Hu},
\authitem{P.~Koch},
\authitem{B.~Kr\"ock},
\authitem{W.~K\"uhn},
\authitem{S.~Lange},
\authitem{Y.~Liang},
\authitem{O.~Merle},
\authitem{V.~Metag},
\authitem{M.~Moritz},
\authitem{D.~M\"unchow},
\authitem{M.~Nanova}, 
\authitem{R.~Novotny},
\authitem{B.~Spruck},
\authitem{H.~Stenzel},
\authitem{T.~Ullrich},
\authitem{M.~Werner},
\authitem{H.~Xu}\lastitem
%
\institem{University of {\bf Glasgow}, United Kingdom}
\authitem{C.~Euan},
\authitem{M.~Hoek},
\authitem{D.~Ireland},
\authitem{T.~Keri},
\authitem{R.~Montgomery},
\authitem{D.~Protopopescu},
\authitem{G.~Rosner},
\authitem{B.~Seitz}\lastitem
%
\institem{Kernfysisch Versneller Instituut, University of {\bf Groningen}, Netherlands}
\authitem{M.~Babai},
\authitem{A.~Glazenborg-Kluttig},
\authitem{M.~Kavatsyuk},
\authitem{P.~Lemmens},
\authitem{M.Lindemulder},
\authitem{H.~L\"ohner},
\authitem{J.~Messchendorp},
\authitem{H.~Moeini},
\authitem{P.~Schakel},
\authitem{F.~Schreuder},
\authitem{H.~Smit},
\authitem{G.~Tambave},
\authitem{J.C. van der Weele},
\authitem{R.~Veenstra}\lastitem
%
\institem{Fachhochschule S\"udwestfalen {\bf Iserlohn}, Germany}
\authitem{H.~Sohlbach}\lastitem
%
\institem{Forschungszentrum J\"ulich, Institut f\"ur Kernphysik, {\bf J\"ulich}, Germany}
\authitem{M.~B\"uscher},
\authitem{D.~Deermann},
\authitem{R.~Dosdall},
\authitem{S.~Esch},
\authitem{A.~Gillitzer},
\authitem{F.~Goldenbaum},
\authitem{D.~Grunwald},
\authitem{S.~Henssler},
\authitem{A.~Herten},
\authitem{Q.~Hu},
\authitem{G.~Kemmerling},
\authitem{H.~Kleines},
\authitem{V.~Kozlov},
\authitem{A.~Lehrach},
\authitem{R.~Maier},
\authitem{M.~Mertens},
\authitem{H.~Ohm},
\authitem{S.~Orfanitski},
\authitem{D.~Prasuhn},
\authitem{T.~Randriamalala},
\authitem{J.~Ritman},
\authitem{S.~Schadmand},
\authitem{V.~Serdyuk},
\authitem{G.~Sterzenbach},
\authitem{T.~Stockmanns},
\authitem{P.~Wintz},
\authitem{P.~W\"ustner},
\authitem{H.~Xu}\lastitem
%
\institem{University of Silesia, {\bf Katowice}, Poland}
\authitem{J.~Kisiel}\lastitem
%
\institem{Chinese Academy of Science, Institute of Modern Physics, {\bf Lanzhou}, China}
\authitem{S.~Li},
\authitem{Z.~Li},
\authitem{Z.~Sun},
\authitem{H.~Xu}\lastitem
%
\institem{INFN Laboratori Nazionali di {\bf Legnaro}, Italy}
\authitem{V.~Rigato}\lastitem
%
\institem{Lunds Universitet, Department of Physics, {\bf Lund}, Sweden}
\authitem{S.~Fissum},
\authitem{K.~Hansen},
\authitem{L.~Isaksson},
\authitem{M.~Lundin},
\authitem{B.~Schr\"oder}\lastitem
%
\institem{Johannes Gutenberg-Universit\"at, Institut f\"ur Kernphysik, {\bf Mainz}, Germany}
\authitem{P.~Achenbach},
\authitem{S.~Bleser},
\authitem{U.~Cahit},
\authitem{M.~Cardinali},
\authitem{A.~Denig},
\authitem{M.~Distler},
\authitem{M.~Fritsch},
\authitem{D.~Kangh},
\authitem{A.~Karavdina},
\authitem{W.~Lauth},
\authitem{H.~Merkel},
\authitem{M.~Michel},
\authitem{M.C.~Mora Espi},
\authitem{U.~M\"uller},
\authitem{J.~Pochodzalla},
\authitem{J.~Prometeusz},
\authitem{S.~Sanchez},
\authitem{A.~Sanchez-Lorente},
\authitem{S.~Schlimme},
\authitem{C.~Sfienti},
\authitem{M.~Thiel},
\authitem{T.~Weber}\lastitem
%
\institem{Research Institute for Nuclear Problems, Belarus State University, {\bf Minsk}, Belarus}
\authitem{V.I.~Dormenev},
\authitem{A.A.~Fedorov},
\authitem{M.V.~Korzhik},
\authitem{O.V.~Missevitch}\lastitem
%
\institem{Institute for Theoretical and Experimental Physics, {\bf Moscow}, Russia}
\authitem{V.~Balanutsa},
\authitem{V.~Chernetsky},
\authitem{A.~Demekhin},
\authitem{A.~Dolgolenko},
\authitem{P.~Fedorets},
\authitem{A.~Gerasimov},
\authitem{V.~Goryachev},
\authitem{V.~Varentsov}\lastitem
%
\institem{Moscow Power Engineering Institute, {\bf Moscow}, Russia}
\authitem{A.~Boukharov},
\authitem{O.~Malyshev},
\authitem{I.~Marishev},
\authitem{A.~Semenov}\lastitem
%
\institem{Technische Universit\"at {\bf M\"unchen}, Germany}
\authitem{F.~B\"ohmer},
\authitem{S.~D$\o$rheim},
\authitem{B.~Ketzer},
\authitem{S.~Paul}\lastitem
%
\institem{Westf\"alische Wilhelms-Universit\"at {\bf M\"unster}, Germany}
\authitem{A.K.~Hergem\"oller},
\authitem{A.~Khoukaz},
\authitem{E.~K\"ohler},
\authitem{A.~T\"aschner},
\authitem{J.~Wessels}\lastitem
%
\institem{IIT Bombay, Department of Physics, {\bf Mumbai}, India}
\authitem{R.~Varma}\lastitem
%
\institem{Bhabha Atomic Research Center, {\bf Mumbai}, India}
\authitem{A.~Chaterjee},
\authitem{V.~Jha},
\authitem{S.~Kailas},
\authitem{B.~Roy}\lastitem
%
\institem{Suranaree University of Technology, {\bf Nakhon Ratchasima}, Thailand}
\authitem{Y.~Yan},
\authitem{K.~Chinorat},
\authitem{K.~Khanchai},
\authitem{L.~Ayut},
\authitem{S.~Pomrad}\lastitem
%
\institem{Budker Institute of Nuclear Physics of Russian Academy of Science, {\bf Novosibirsk}, Russia}
\authitem{E.~Baldin},
\authitem{K.~Kotov},
\authitem{S.~Peleganchuk},
\authitem{Yu.~Tikhonov}\lastitem
%
\institem{Institut de Physique Nucl\'{e}aire, {\bf Orsay}, France}
\authitem{J.~Boucher},
\authitem{V.~Chambert},
\authitem{A.~Dbeyssi},
\authitem{T.~Hennino},
\authitem{M.~Imre},
\authitem{R.~Kunne},
\authitem{C.~Le~Galliard},
\authitem{B.~Ma},
\authitem{D.~Marchand},
\authitem{A.~Maroni},
\authitem{S.~Ong},
\authitem{B.~Ramstein},
\authitem{P.~Rosier},
\authitem{M.~Sudol},
\authitem{E.~Tomasi-Gustafsson},
\authitem{J.~Van~de~Wiele}\lastitem
%
\institem{Dipartimento di Fisica Nucleare e Teorica, Universit\`{a} di Pavia, 
INFN Sezione di Pavia, {\bf Pavia}, Italy}
\authitem{G.~Boca},
\authitem{A.~Braghieri},
\authitem{S.~Costanza},
\authitem{P.~Genova},
\authitem{L.~Lavezzi},
\authitem{P.~Montagna},
\authitem{A.~Rotondi}\lastitem
%
\institem{Institute for High Energy Physics, {\bf Protvino}, Russia}
\authitem{V.~Abramov},
\authitem{N.~Belikov},
\authitem{A.~Davidenko},
\authitem{A.~Derevschikov}, 
\authitem{Y.~Goncharenko},
\authitem{V.~Grishin}, 
\authitem{V.~Kachanov},
\authitem{D.~Konstantinov}, 
\authitem{V.~Kormilitsin},
\authitem{Y.~Melnik},
\authitem{A.~Levin},
\authitem{N.~Minaev}, 
\authitem{V.~Mochalov}, 
\authitem{D.~Morozov}, 
\authitem{L.~Nogach}, 
\authitem{S.~Poslavskiy}, 
\authitem{A.~Ryazantsev},
\authitem{S.~Ryzhikov},
\authitem{P.~Semenov},
\authitem{I.~Shein},
\authitem{A.~Uzunian},
\authitem{A.~Vasiliev},
\authitem{A.~Yakutin}\lastitem
%
\institem{Kungliga Tekniska H\"ogskolan, {\bf Stockholm}, Sweden}
\authitem{T.~B\"ack},
\authitem{B.~Cederwall}\lastitem
%
\institem{Stockholms Universitet, {\bf Stockholm}, Sweden}
\authitem{K.~Mak\'onyi},
\authitem{P.E.~Tegn\'{e}r},
\authitem{K.M.~von W\"urtemberg}\lastitem
%
\institem{Petersburg Nuclear Physics Institute of Russian Academy of Science,
Gatchina, {\bf St.~Petersburg}, Russia}
\authitem{S.~Belostotski},
\authitem{G.~Gavrilov},
\authitem{A.~Itzotov},
\authitem{A.~Kashchuk},
\authitem{A.~Kisselev},
\authitem{P.~Kravchenko},
\authitem{O.~Levitskaya},
\authitem{S.~Manaenkov},
\authitem{O.~Miklukho},
\authitem{Y.~Naryshkin},
\authitem{D.~Veretennikov},
\authitem{V.~Vikhrov},
\authitem{A.~Zhadanov}\lastitem
%
\institem{Universit\`{a} di Torino and INFN Sezione di~Torino, {\bf Torino}, Italy}
\authitem{D.~Alberto}, 
\authitem{A.~Amoroso},
\authitem{M.P.~Bussa},
\authitem{L.~Busso}, 
\authitem{F.~De Mori},
\authitem{M.~Destefanis},
\authitem{L.~Fava},
\authitem{L.~Ferrero},
\authitem{M.~Greco}, 
\authitem{M.~Maggiora},
\authitem{S.~Marcello},
\authitem{S.~Sosio},
\authitem{S.~Spataro},
\authitem{L.~Zotti}
\lastitem
%
\institem{INFN Sezione di~Torino, {\bf Torino}, Italy}
\authitem{D.~Calvo},
\authitem{S.~Coli},
\authitem{P.~De~Remigis},
\authitem{A.~Filippi},
\authitem{G.~Giraudo},
\authitem{S.~Lusso},
\authitem{G.~Mazza},
\authitem{O.~Morra},
\authitem{A.~Rivetti},
\authitem{R.~Wheadon}\lastitem
%
\institem{Politecnico di Torino and INFN Sezione di~Torino,{\bf Torino}, Italy}
\authitem{F.~Iazzi},
\authitem{A.~Lavagno},
\authitem{H.~Younis}\lastitem
%
\institem{Universit\`{a} di Trieste and INFN Sezione di Trieste, {\bf Trieste}, Italy}
\authitem{R.~Birsa},
\authitem{F.~Bradamante},
\authitem{A.~Bressan},
\authitem{A.~Martin}\lastitem
%
\institem{Universit\"at T\"ubingen, {\bf T\"ubingen}, Germany}
\authitem{H.~Clement}\lastitem
%
\institem{The Svedberg Laboratory, {\bf Uppsala}, Sweden}
\authitem{B.~Galander}\lastitem
%
\institem{Uppsala Universitet, Institutionen f\"or Str\aa lningsvetenskap, {\bf Uppsala}, Sweden}
\authitem{L.~Caldeira Balkest{\aa}hl},
\authitem{H.~Cal\'en},
\authitem{K.~Fransson},
\authitem{T.~Johansson},
\authitem{A.~Kupsc},
\authitem{P.~Marciniewski},
\authitem{E.~Thom\'e},
\authitem{M.~Wolke},
\authitem{J.~Zlomanczuk}\lastitem
%
\institem{Universitat de {\bf Valencia}, Dpto. de F\'isica At\'omica, Molecular y Nuclear, Spain}
\authitem{J.~D\'iaz},
\authitem{A.~Ortiz}\lastitem
%
\institem{University of Technology, Institute of Atomic Energy Otwock-Swierk, {\bf Warsaw}, Poland}
\authitem{K.~Dmowski},
\authitem{P.~Duda},
\authitem{R.~Korzeniewski},
\authitem{B.~Slowinski}\lastitem
%
\institem{National Centre for Nuclear Research, {\bf Warsaw}, Poland}
\authitem{A.~Chlopik},
\authitem{Z.~Guzik},
\authitem{K.~Kosinski},
\authitem{D.~Melnychuk},
\authitem{A.~Wasilewski},
\authitem{M.~Wojciechowski},
\authitem{S.~Wronka},
\authitem{A.~Wysocka},
\authitem{B.~Zwieglinski}\lastitem
%
\institem{\"Osterreichische Akademie der Wissenschaften, Stefan Meyer Institut f\"ur Subatomare Physik, {\bf Wien}, Austria}
\authitem{P.~B\"uhler},
\authitem{O.~Hartman},
\authitem{P.~Kienle},
\authitem{J.~Marton},
\authitem{K.~Suzuki},
\authitem{E.~Widmann},
\authitem{J.~Zmeskal}\lastitem
%\centerline{$^\dagger$\ Membership to be approved by the Coordination Board}
%
% EOF
%


==> panda_tdr_stt.tex <==
%
% Panda TDR 
% Main File for STT TDR
\cleardoublepage
\setcounter{chapter}{1}
\input{panda_stt_cp1}
\input{panda_stt_cp2}
\input{panda_stt_cp3}
\input{panda_stt_cp4}
\input{panda_stt_cp5}
\input{panda_stt_cp6}
\input{panda_stt_cp7}
\input{panda_stt_cp8}
%
% Bibliography for this chapter (remove %)
%
\newpage
%\bibliographystyle{panda_tdr_lit}
%\bibliography{./stt/lit_stt}
% EOF


==> panda_tdr_trk_req.tex <==
% FILE: panda_tdr_trk_req.tex
%
% PANDA STT TDR
% Main File for Chapter
%''Overview of the project and the requirements''
%
\cleardoublepage
\chapter{Overview of the project and the requirements}
\label{sec:req}
%
% Text for this section
%
\input{./req/req.tex}
%
% Bibliography for this chapter (remove %)
%
\newpage
\bibliographystyle{panda_tdr_lit}
\bibliography{./lit_trk}
%
% EOF: panda_tdr_trk_req.tex


==> sty/panda_commands.tex <==
% def_panda_cmd.tex
%
\RequirePackage[centertags]{amsmath}
%
\RequirePackage{xspace}
%\RequirePackage{ulem}
%
\def\MARK#1{\texorpdfstring{{\emph{\textcolor{red}{#1}}}}{{#1}}}
%\def\MARK#1{\emph{\textcolor{red}{#1}}}
%\def\MARK#1{{\bf \textcolor{red}{#1}}}
%\def\MARK#1{{#1}}
% use to mark text 
% (Text will be kept, but the marking removed in the final document)
%
\def\COM#1{\fbox{\parbox{\swidth}{\textcolor{red}{\bf COMMENT: #1}}}}
%\def\COM#1{}
% use to add comments
% (The whole will be removed in the final version)
%
% use to mark parts, which shouldn't be present in the cost-free version

\def\OnlyLayoutColumnBreak{{\vfill\newpage}}%

\def\OnlyLayoutPageBreak{{\vfill\clearpage}}%

\def\OnlyLayoutDoublePageBreak{{\vfill\cleardoublepage}}%

%
\def\bfg{\begin{figure}}%
\def\efg{\end{figure}}%
\def\bc{\begin{center}}%
\def\ec{\end{center}}%
\def\bi{\begin{itemize}}%
\def\ei{\end{itemize}}%
\def\beq{\begin{equation}}%
\def\eeq{\end{equation}}%
\def\bn{\begin{eqnarray}}%
\def\en{\end{eqnarray}}%
\def\ba#1{\left(\begin{array}{#1}}%
\def\ea{\end{array}\right)}%
\def\bef{\begin{equation}\fbox{$\displaystyle}%
\def\eef{$}\end{equation}}%
\def\bnf{\bef\ba{rcl}}%
\def\enf{\ea\eef}%
\newcommand{\beal}{\begin{align}}
\newcommand{\eal}{\end{align}}
\newcommand{\bespl}{\begin{split}}
\newcommand{\espl}{\end{split}}
%\def\refeq#1{\Eqref{#1}\xspace}%
%\def\Refsec#1{sec.~\ref{#1}\xspace}%
%\def\Refchap#1{\Refchap{#1}\xspace}%
%\def\Reffig#1{\Reffig{#1}\xspace}%
%\def\Reftbl#1{\Reftbl{#1}\xspace}%
%\def\reftab#1{\Reftbl{#1}\xspace}%
\def\Refeq#1{Eq.~\ref{#1}\xspace}%
\def\Refeqs#1{Eqs.~\ref{#1}\xspace}%
\def\Refsec#1{Sec.~\ref{#1}\xspace}%
\def\Refchap#1{Chap.~\ref{#1}\xspace}%
\def\Reffig#1{Fig.~\ref{#1}\xspace}%
\def\Reffigs#1{Figs.~\ref{#1}\xspace}%
\def\Reftbl#1{Table~\ref{#1}\xspace}%
\def\Reftbls#1{Tables~\ref{#1}\xspace}%
\def\RefeqX#1{Eq.~\ref{#1}}%
\def\RefeqsX#1{Eqs.~\ref{#1}}%
\def\RefsecX#1{Sec.~\ref{#1}}%
\def\RefchapX#1{Chap.~\ref{#1}}%
\def\ReffigX#1{Fig.~\ref{#1}}%
\def\ReffigsX#1{Figs.~\ref{#1}}%
\def\ReftblX#1{Table~\ref{#1}}%
\def\ReftblsX#1{Tables~\ref{#1}}%
%\def\Reftab#1{Table~\ref{#1}\xspace}%
\def\ub{\underbrace}%
%
\def\vps{\hspace*{5mm}}%
\def\dsty{\displaystyle}%
%
\newcounter{auth}%
\setcounter{auth}{0}%
\def\authitem#1{\addtocounter{auth}{1}#1}%
\def\authitemi#1#2{\addtocounter{auth}{1}#2$^{#1}$}%
\newcounter{inst}%
\setcounter{inst}{0}%
\def\institem#1{\par \addtocounter{inst}{1}#1\\}%
\def\lastitem{\ }%
\def\respitem#1{\institem{{\bf #1}\lastitem\\}}%
\let\groupitem=\authitem
%
\newcommand{\captionfonts}{\small}
%
\makeatletter  % Allow the use of @ in command names
\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip
  \sbox\@tempboxa{{\captionfonts {\bf #1:} #2}}%
  \ifdim \wd\@tempboxa >\hsize
    {\captionfonts {\bf #1:} #2\par}
  \else
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}
\makeatother   % Cancel the effect of \makeatletter
%
% a few commands to change the figure placing (commented are the default values)
%\renewcommand{\textfraction}{0.1} % 0.2
%\renewcommand{\bottomfraction}{0.4} % 0.3
%\renewcommand{\dbltopfraction}{0.8} % 0.7
%\renewcommand{\dblfloatpagefraction}{0.3} % 0.5
%\renewcommand{\floatpagefraction}{0.3} % 0.5
%\setcounter{dbltopnumber}{3} % 2
%\setcounter{bottomnumber}{2} % 1
%
\def\markpanda#1#2{\markboth{\Panda{} - #1}{FAIR/Pbar/#2}}%
%
\newcommand{\unit}[1]{\,\mathrm{#1}}

% EOF: def_panda_cmd.tex


==> sty/panda_detector.tex <==
% panda_detector.tex
%
\RequirePackage{xspace}
%
\def\INST#1{\texorpdfstring{{\sffamily #1}}{{#1}}\xspace}%
%
\def\PANDA{\texorpdfstring{$\overline{\mbox{\sffamily P}}${\sffamily ANDA}}{Panda}\xspace}%
\def\Panda{\texorpdfstring{$\overline{\mbox{\sffamily P}}${\sffamily ANDA}}{Panda}\xspace}%
\def\panda{\texorpdfstring{$\overline{\mbox{\sffamily P}}${\sffamily ANDA}}{Panda}\xspace}%
\def\HESR{\INST{HESR}}%
\def\Hesr{\INST{HESR}}%
\def\GSI{\INST{GSI}}%
\def\Gsi{\INST{GSI}}%
\def\FAIR{\INST{FAIR}}%
\def\Fair{\INST{FAIR}}%
%
% General definitions
%
\def\Ts{TS\xspace}
\def\Fs{FS\xspace}
\def\Mvd{MVD\xspace}
\def\Emc{EMC\xspace}
\def\TsEmc{TS-EMC\xspace}
\def\FsEmc{FS-EMC\xspace}
\def\Had{HAD\xspace}
\def\Muo{MUO\xspace}
\def\TsMuo{TS-MUO\xspace}
\def\FsMuo{FS-MUO\xspace}
\def\Stt{STT\xspace}
\def\Tpc{TPC\xspace}
\def\Dirc{DIRC\xspace}
\def\Rich{RICH\xspace}
\def\Mdc{MDC\xspace}
\def\TsMdc{TS-MDC\xspace}
\def\FsMdc{FS-MDC\xspace}
\def\Tof{TOF\xspace}
\def\Lum{LUM\xspace}
\def\Mag{MAG\xspace}
\def\TsMag{SOL\xspace}
\def\FsMag{DIP\xspace}
%
% EMC definitions
%
\def\BEMC{barrel EMC\xspace}
\def\FWEMC{forward endcap EMC\xspace}
\def\BWEMC{backward endcap EMC\xspace}
\def\TSEMC{target spectrometer EMC\xspace}
\def\FSEMC{forward spectrometer EMC\xspace}
\def\TsEmc{\TSEMC}
\def\FsEmc{\FSEMC}
%
\def\LAAPD{LAAPD\xspace}
\def\LAAPDs{LAAPDs\xspace}
\def\VPT{VPT\xspace}
\def\VPTs{VPTs\xspace}
\def\PWOII{PWO-II\xspace}
\def\PWO{PWO\xspace}

% EOF: def_panda_det.tex


==> sty/panda_symbols.tex <==
% def_panda_sym.tex
%
\input{./sty/pennames.sty}
\input{./sty/myunits.sty}
\input{./sty/mymath.sty}
%
\RequirePackage{xspace}
% Upright mu for micro
\DeclareFontFamily{U}{euc}{}% I chose euc because the chart is called Euler cursive
\DeclareFontShape{U}{euc}{m}{n}{<-6>eurm5<6-8>eurm7<8->eurm10}{}%
\DeclareSymbolFont{AMSc}{U}{euc}{m}{n} % I chose AMSc because AMSa and AMSb are defined in the amsfonts-package
\DeclareMathSymbol{\umu}{\mathord}{AMSc}{"16}
%
\def\degrees{\ensuremath{^\circ}\xspace}%
\def\percent{$\,$\%\xspace}%
\def\prm{\ensuremath{^\prime}}%
\def\etc{{\em etc.}\xspace}%
% Andreas's
\newcommand{\q}[2]{\ensuremath{#1\ \mathrm{#2}}}
\newcommand{\eperp}{\ensuremath{\varepsilon_\perp}}
\newcommand{\stot}{\ensuremath{\sigma_\mathrm{tot}}}
\newcommand{\tauloss}{\ensuremath{\tau_\mathrm{loss}}}
\newcommand{\tpbar}{\ensuremath{t_{\bar{p}}}}
\newcommand{\Lmax}{\ensuremath{L_\mathrm{max}}}
\newcommand{\Npbar}{\ensuremath{N_{\bar{p}}}}
\newcommand{\tprep}{\ensuremath{t_\mathrm{prep}}}
\newcommand{\texp}{\ensuremath{t_\mathrm{exp}}}
\newcommand{\tcycle}{\ensuremath{t_\mathrm{cycle}}}
%
% theory stuff
%
\newcommand{\MZ}{M^{\!\!\!\!\!^o}}
\newcommand{\aslash}{\FMslash a}
\newcommand{\Partialslash}{\FMslash \partial}
\newcommand{\vslash}{\FMslash v}
\newcommand{\pslash}{\FMslash p}
\newcommand{\wslash}{\FMslash w}
\newcommand{\lslash}{\FMslash l}
\newcommand{\Lslash}{\FMslash L}
\newcommand{\qslash}{\FMslash q}
\newcommand{\Qslash}{\FMslash Q}
\newcommand{\Pslash}{\FMslash P}
\newcommand{\Wslash}{\FMslash W}
\newcommand{\kslash}{\FMslash k}
\newcommand{\Kslash}{\FMslash K}
\newcommand{\barKslash}{\FMslash {\bar K}}
\newcommand{\barPslash}{\FMslash {\bar P}}
\newcommand{\kapslash }{\FMslash \kappa }
\newcommand{\chiral}[1]{\stackrel{\circ}{#1}}
\def\Re{{\rm Re\,}}
\def\Im{{\rm Im\,}}
\def\prt{\partial}
%
\def\BW{\ensuremath{\mbox{\it BW}}\xspace}%
\def\BR{\ensuremath{\mathcal{B}}\xspace}%
\def\LH{\ensuremath{\mathcal{L}}\xspace}%
\def\CL{\ensuremath{\mbox{\it CL}}\xspace}%
%
\def\vloo{\mbox{\tt VeryLoose}\xspace}
\def\loo{\mbox{\tt Loose}\xspace}
\def\tig{\mbox{\tt Tight}\xspace}
\def\vtig{\mbox{\tt Tight}\xspace}
%
\def\tm{\texttrademark}
\def\tmr{\ensuremath{^{\textregistered}}}
%
\def\ppbar{\ensuremath{\mbox{p}\overline{\mbox{p}}}\xspace}%
\def\pbarp{\ensuremath{\overline{\mbox{p}}\mbox{p}}\xspace}%
\def\NNbar{\ensuremath{N\overline{N}}\xspace}%
\def\pbard{\ensuremath{\overline{\mbox{p}}\mbox{d}}\xspace}%
\def\pbarA{\ensuremath{\overline{\mbox{p}}\mbox{A}}\xspace}%
\def\pbarN{\ensuremath{\overline{\mbox{p}}\mbox{N}}\xspace}%
\def\pbard{\ensuremath{\overline{\mbox{p}}\mbox{d}}\xspace}%
\def\pbar{\ensuremath{\overline{\mbox{p}}}\xspace}%s
\def\nbar{\ensuremath{\overline{\mbox{n}}}\xspace}%
\def\pbarn{\ensuremath{\overline{\mbox{p}}\mbox{n}}\xspace}%
\def\nbarn{\ensuremath{\overline{\mbox{n}}\mbox{n}}\xspace}%
\def\NbarN{\ensuremath{\overline{N}N}\xspace}%
%
\def\qbar{\ensuremath{\overline{q}}\xspace}%
\def\cbar{\ensuremath{\overline{c}}\xspace}%
\def\ccbar{\ensuremath{c\overline{c}}\xspace}%
\def\ccbarg{\ensuremath{c\overline{c}g}\xspace}%
\def\cqbar{\ensuremath{c\overline{q}}\xspace}%
\def\cbarq{\ensuremath{\overline{c}q}\xspace}%
\def\uubar{\ensuremath{u\overline{u}}\xspace}%
\def\ddbar{\ensuremath{d\overline{d}}\xspace}%
\def\ssbar{\ensuremath{s\overline{s}}\xspace}%
\def\bbbar{\ensuremath{b\overline{b}}\xspace}%
\def\bqbar{\ensuremath{b\overline{q}}\xspace}%
\def\bbarq{\ensuremath{\overline{b}q}\xspace}%
\def\qqbar{\ensuremath{q\overline{q}}\xspace}%
\def\qqbarg{\ensuremath{q\overline{q}g}\xspace}%
\def\QQbar{\ensuremath{Q\overline{Q}}\xspace}%
%
\def\ee{\ensuremath{e^+e^-}\xspace}%
\def\mumu{\ensuremath{\mu^+\mu^-}\xspace}%
%
\def\piz{\ensuremath{\pi^0}\xspace}%
\def\pip{\ensuremath{\pi^+}\xspace}%
\def\pim{\ensuremath{\pi^-}\xspace}%
\def\pipm{\ensuremath{\pi^\pm}\xspace}%
\def\pimp{\ensuremath{\pi^\mp}\xspace}%
%
\def\K{\ensuremath{K}\xspace}%
\def\Kp{\ensuremath{K^+}\xspace}%
\def\Km{\ensuremath{K^-}\xspace}%
\def\Kpm{\ensuremath{K^\pm}\xspace}%
\def\Kmp{\ensuremath{K^\mp}\xspace}%
\def\KKbar{\ensuremath{K\overline{K}}\xspace}%
\def\Kz{\ensuremath{K^0}\xspace}%
\def\Kbar{\ensuremath{\overline{K}}\xspace}%
\def\Kzbar{\ensuremath{\overline{K}^0}\xspace}%
\def\KzKzbar{\ensuremath{K^0\overline{K^0}}\xspace}%
\def\Ks{\ensuremath{K_S^0}\xspace}%
\def\Kl{\ensuremath{K_L^0}\xspace}%
%
\def\etaprime{\ensuremath{\eta\prm}\xspace}%
\def\pione{\ensuremath{\pi_1}\xspace}%
%
\def\uquark{\ensuremath{u}\xspace}%
\def\dquark{\ensuremath{d}\xspace}%
\def\squark{\ensuremath{s}\xspace}%
\def\cquark{\ensuremath{c}\xspace}%
\def\bquark{\ensuremath{b}\xspace}%
\def\tquark{\ensuremath{t}\xspace}%
%
\def\D{\ensuremath{D}\xspace}%
\def\Dbar{\ensuremath{\overline{D}}\xspace}%
\def\DDbar{\ensuremath{D\overline{D}}\xspace}%
\def\DpDm{\ensuremath{D^+D^-}\xspace}%
\def\Dz{\ensuremath{D^0}\xspace}%
\def\Dzbar{\ensuremath{\overline{D}^0}\xspace}%
\def\DzDzbar{\ensuremath{D^0\overline{D}^0}\xspace}%
\def\DzDzxbar{\ensuremath{D^0\overline{D}^{\ast0}}\xspace}%
\def\Dx{\ensuremath{D^\ast}\xspace}%
\def\Dxbar{\ensuremath{\overline{D}^\ast}\xspace}%
\def\DxDxbar{\ensuremath{D^\ast\overline{D}^\ast}\xspace}%
\def\Dxz{\ensuremath{D^{\ast 0}}\xspace}%
\def\Dxzbar{\ensuremath{\overline{D}^{\ast 0}}\xspace}%
\def\DbarDxx{\ensuremath{D\overline{D}^{\ast\ast}}\xspace}%
%
\def\Ds{\ensuremath{D_s}\xspace}%
\def\Dspm{\ensuremath{D_s^\pm}\xspace}%
\def\Dsmp{\ensuremath{D_s^\mp}\xspace}%
\def\Dsx{\ensuremath{D_s^\ast}\xspace}%
\def\Dsxpm{\ensuremath{D_s^{\ast\pm}}\xspace}%
\def\Dsxmp{\ensuremath{D_s^{\ast\mp}}\xspace}%
\def\DsDsbar{\ensuremath{D_s\overline{D_s}}\xspace}%
\def\DspDsm{\ensuremath{D_s^+D_s^-}\xspace}%
\def\DsxDsxbar{\ensuremath{D_s^\ast\overline{D_s}^\ast}\xspace}%
\def\DsbarDsxx{\ensuremath{\overline{D_s}D_s^{\ast\ast}}\xspace}%
%
\def\jpsi{\ensuremath{J\!/\!\psi}\xspace}%
\def\psiprime{\ensuremath{\psi\prm}\xspace}%
\def\etac{\ensuremath{\eta_c}\xspace}%
\def\etacprime{\ensuremath{\eta\prm_c}\xspace}%
\def\chicJ{\ensuremath{\chi_{cJ}}\xspace}%
\def\chiczero{\ensuremath{\chi_{c0}}\xspace}%
\def\chicone{\ensuremath{\chi_{c1}}\xspace}%
\def\chictwo{{\chi_{c2}}\xspace}%
\def\honec{\ensuremath{h_c}\xspace}%
%
\def\Cascade{\ensuremath{\Xi}\xspace}%
\def\Cascadebar{\ensuremath{\overline{\Xi}}\xspace}%
\def\Lambdabar{\ensuremath{\overline{\Lambda}}\xspace}%
\def\LambdaLambdabar{\ensuremath{\Lambda\overline{\Lambda}}\xspace}%
\def\Omegabar{\ensuremath{\overline{\Omega}}\xspace}%
\def\OmegaOmegabar{\ensuremath{\Omega\overline{\Omega}}\xspace}%
\def\Sigmabar{\ensuremath{\overline{\Sigma}}\xspace}%
\def\SigmaSigmabar{\ensuremath{\Sigma\overline{\Sigma}}\xspace}%
\def\CascadeCascadebar{\ensuremath{\Xi\overline{\Xi}}\xspace}%
\def\Lambdac{\ensuremath{\Lambda_c}\xspace}%
\def\Sigmac{\ensuremath{\Sigma_c}\xspace}%
\def\Omegac{\ensuremath{\Omega_c}\xspace}%
\def\Cascadec{\ensuremath{\Xi_c}\xspace}%
%
\def\kev{{\mbox{keV}}\xspace}%
\def\kevcc{{\mbox{keV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\mev{{\mbox{MeV}}\xspace}%
\def\mevc{{\mbox{MeV}\!/\!\mbox{\em c}}\xspace}%
\def\mevcc{{\mbox{MeV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\mevccsq{{\mbox{MeV$^2$}\!/\!\mbox{\em c$^4$}}\xspace}%
\def\gev{{\mbox{GeV}}\xspace}%
\def\gevc{{\mbox{GeV}\!/\!\mbox{\em c}}\xspace}%
\def\gevcsq{{\mbox{GeV$^2$}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\gevcc{{\mbox{GeV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\gevccsq{{\mbox{GeV$^2$}\!/\!\mbox{\em c$^4$}}\xspace}%
%
\def\aC{{\mbox{aC}}\xspace}%
%
\def\barn{\ensuremath{\rm \,b}\xspace}
\def\barnhyph{\ensuremath{\rm -b}\xspace}
\def\mbarn{\ensuremath{\rm \,mb}\xspace}
\def\mbarnhyph{\ensuremath{\rm -mb}\xspace}
\def\mubarn{\ensuremath{\rm \,\mu b}\xspace}
\def\nb{\ensuremath{\rm \,nb}\xspace}
\def\pb {\ensuremath{\rm \,pb}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
%
\def\JPC{\ensuremath{J^{\!P\!C}}\xspace}%
\def\JPCzeropm{\ensuremath{0^{+-}}\xspace}%
\def\JPCzeropp{\ensuremath{0^{++}}\xspace}%
\def\JPCzeromm{\ensuremath{0^{--}}\xspace}%
\def\JPCzeromp{\ensuremath{0^{-+}}\xspace}%
\def\JPConepm{\ensuremath{1^{+-}}\xspace}%
\def\JPConepp{\ensuremath{1^{++}}\xspace}%
\def\JPConemm{\ensuremath{1^{--}}\xspace}%
\def\JPConemp{\ensuremath{1^{-+}}\xspace}%
\def\JPCtwopm{\ensuremath{2^{+-}}\xspace}%
\def\JPCtwopp{\ensuremath{2^{++}}\xspace}%
\def\JPCtwomm{\ensuremath{2^{--}}\xspace}%
\def\JPCtwomp{\ensuremath{2^{-+}}\xspace}%
%
\def\JPCscalar{\JPCzeropp}%
\def\JPCvector{\JPConemm}%
\def\JPCtensor{\JPCtwopp}%
%
\def\GE {\relax\ifmmode{\rm G_E}%
         \else${\rm G_E}$\fi}
\def\GM {\relax\ifmmode{\rm G_M}%
         \else${\rm G_M}$\fi}
\def\Fi {\relax\ifmmode{\rm F_1}%
         \else${\rm F_1}$\fi}
\def\Fii {\relax\ifmmode{\rm F_2}%
         \else${\rm F_1}$\fi}
\def\qsq {\relax\ifmmode{\rm q^2}%
         \else${\rm q^2}$\fi}
%
\def\tO{\,\rightarrow\,}
%
\def\extl{\ensuremath{E_{xtl}}\xspace}
\def\ecl{\ensuremath{E_{cl}}\xspace}
\def\emax{\ensuremath{E_{max}}\xspace}
%
% Simulation symbols
\def\pandaroot{\texttt{PandaRoot}\xspace}%
\def\fairroot{\texttt{FairRoot}\xspace}%
\def\pandagrid{\texttt{PandaGrid}\xspace}%
% EOF: def_panda_sym.tex

